SimpleDG: Simple Domain Generalization Baseline without Bells and Whistles

We present a simple domain generalization baseline, which wins second place in both the common context generalization track and the hybrid context generalization track respectively in NICO CHALLENGE 2022. We verify the founding in recent literature, domainbed, that ERM is a strong baseline compared to recent state-of-the-art domain generalization methods and propose SimpleDG which includes several simple yet effective designs that further boost generalization performance. Code is available at https://github.com/megvii-research/SimpleDG

==> discussion.tex <==






% \begin{figure}[htp]
%   \centering
% %   \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
% \includegraphics[width=1.0\textwidth]{figs/cam_llz_eccv1.png}
%   \caption{CAM~\cite{zhou2016learning} visualization on ImageNet and INAT21. Our method focuses more on the correct object consistent with the prediction instead of relying on irrelevant objects from the backgrounds.}
%   \label{fig:cam}
% \end{figure}



% In this section, we would go to detail analysis about soft distribution generated by our method and its effects, such as feature space and CAM visualization.
% \noindent \textbf{SNR of ranking during  training}
% We first examine SNR of ranking over all samples in INAT dataset. Signal is defined as average value of sorted value among samples of the same rank, and  noise is defined as standard deviation of sorted value among samples of the same rank. See Fig. \ref{fig:snr}, larger the rank is, lower the SNR is, and only little small fraction of head class, 30 in this case, the SNR of the rank is larger than 1. To add different epoch result.

\noindent \textbf{Zipf's soft labels results in more reasonable predictions.} Fig.~\ref{fig:result_sample} illustrates the top-5 predictions of our proposed method compared with the baseline method. The images are sampled from ImageNet and INAT21 respectively. Our method makes more reasonable predictions. Not only the top-1 prediction is correct, but also more similar concepts arise in the top-5 prediction. This results from more informative soft labels from Zipf's LS, which provides meaningful representations as knowledge distillation for the network to better grasp the concept of similar categories.
\begin{figure*}[t]
  \centering
%   \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
\includegraphics[width=1.\textwidth]{figs/feature_distributions_150x150.png}
  \caption{T-SNE~\cite{van2008visualizing} visualization on 50 random sampled classes of TinyImageNet for CE, Label Smoothing and Zipf's label smoothing.}
  \label{fig:feature_vis}
\end{figure*}

\setlength{\tabcolsep}{4pt}
\begin{table}[!htp]\centering
\caption{Comparison of the top-1 accuracy (\%) of different distributions and label smoothing. Experiments are conducted on TinyImageNet, ImageNet and INAT21. Zipf makes the best performance among these distributions}\label{tab: 6}
\scriptsize
\begin{tabular}{lcccc}\toprule
\textbf{Distribution} &\textbf{TinyImageNet} &\textbf{ImageNet} &\textbf{INAT21} \\\cmidrule{1-4}
Vanilla &56.41 &76.48 &62.43 \\ \cmidrule{1-4}
LS &56.89 &76.67 &65.16 \\
Constant &58.76 &77.09 &65.86 \\
Random\_Uniform &58.24 &76.89 &65.61\\
Random\_Pareto &58.52 &76.61 &65.9\\
Linear\_Decay &58.39 &76.87 &65.86\\\cmidrule{1-4}
Zipf &\textbf{59.25} &\textbf{77.25} &\textbf{66.04}\\ 
\bottomrule
\end{tabular}
\end{table}
\setlength{\tabcolsep}{1.4pt}


\noindent \textbf{Zipf's Label Smoothing achieves better representation learning for generalization.} We compare our Zipf's LS techniques with  cross-entropy training and uniform label smoothing training on the TinyImageNet dataset. As shown in Fig.~\ref{fig:feature_vis}, the intra-class distance in feature space learned from Zipf's label smoothing is more compact and the inter-class distance is more separate. Zipf's Label Smoothing achieves better representation learning for generalization. More discussion for generalization is shown in supplements.

\noindent \textbf{Non-target class dense classification ranking design.} To better rank the classes in the soft label, we exploit dense classification ranking instead of logits-based ranking. Thus, larger objects are favored and small object classification performance might degrade. In our design, the target class is excluded in $L_{Zipf}$ and included in $L_{CE}$ only, ensuring the target class provides the correct gradient regardless of the object size. To verify the small object performance, we collect the five smallest objects from each class\footnote{\url{https://image-net.org/data/bboxes_annotations.tar.gz}}, Zipf's LS still beat CE(69.25\% vs 67.72\%). The cam visualization for the small object case is shown in Fig \ref{fig:small_objects}

% \noindent \textbf{Further discussions and explanations of our method's factors.} Here we conclude and try to explain the reasons for the effectiveness of our method. Firstly, it's important to design the ranking distribution law on non-target classes but not all classes. Table \ref{tab: 6} shows constant distribution which means using non-target strategy on label smoothing outperforms original label smoothing. Non-target strategy prevents the distillation optimization task from the dominating of target class. Secondly, dense classification ranking helps performance on low resolution, while logits-based ranking strategy shows advantages on small objects. We collect five most smallest objects from each class\footnote{\url{image-net.org/data/bboxes_annotations.tar.gz}}, Zipf's LS achieve better performance(69.25\% vs 67.72\%). The cam visualization is shown in Fig \ref{fig:small_objects}. Our method encourages large objects competition in non-target class, which shall encourage more robust representation learning for small objects in target class to make the correct prediction. Thirdly, we propose an experiment to verify that softmax Gaussian logits fit Zipf’s law well in supplement, which empirically explains why Zipf's law could help generate better supervision compared with other frequently-used distribution.

\begin{figure*}[t]
  \centering
%   \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
\includegraphics[width=1\textwidth]{figs/small_object.png}
  \caption{Comparison of small objects results between CE(above) and Zipf's LS(below).}
  \label{fig:small_objects}
\end{figure*}


% \noindent \textbf{Feature space and CAM visualization compared with baseline methods.} We compare our Zipf's Label Smoothing techniques with two baseline methods, cross-entropy training and uniform label smoothing training on TinyImageNet dataset. As shown in Figure~\ref{fig:feature_vis}, the intra-class distance in feature space learned from Zipf's label smoothing is more compact than that of baselines and the inter-class distance is more separate. In CAM visualization~\cite{zhou2016learning}, as shown in Figure.~\ref{fig:cam} our method focuses more on the correct object consistent with the prediction instead of relying on irrelevant objects from the backgrounds, which benefits from the regularized soft labels voted from dense classification.

\noindent \textbf{Limitation.} Zipf's LS does not help in binary classification cases, since the $L_{zipf}$ only considers non-target class and would always be zero. Further, as mentioned in the method section, we exploit dense classification ranking to get more reliable ranking information than logit-based ranking, which is only available in image data but not in modals such as speech and language. To make Zipf's LS work in multi-modal data is considered as future work.   



% \noindent \textbf{rank SNR}
% show rank example and rank SNR compare

% \noindent \textbf{feature visualize}
% cam and low-dimension visualize

% \noindent \textbf{fine-grained improvement}

==> method.tex <==




% \begin{algorithm}[h]
% \SetAlgoLined
%     %\Pycode{
%     % \Indp
%     % m = len(genl1) \\
%     % n = len(genl2) \\
%     % M = None \PyComment{to become the incidence matrix} \\
%     % VT = np.zeros((n*m,1), int)  \PyComment{dummy variable} \\
    
%     % \PyComment{compute the bitwise xor matrix} \\
%     % M1 = bitxormatrix(genl1) \\ 
%     % M2 = np.triu(bitxormatrix(genl2),1) \\

%     % for i in range(m-1): \\
%     % \Indp
%     %     for j in range(i+1, m): \\
%     %         [r,c] = np.where(M2 == M1[i,j]) \\
%     %         for k in range(len(r)): \\
%     %             VT[(i)*n + r[k]] = 1; \\
%     %             VT[(i)*n + c[k]] = 1; \\
%     %             VT[(j)*n + r[k]] = 1; \\
%     %             VT[(j)*n + c[k]] = 1; \\
                
%     %             if M is None: \\
%     %                 M = np.copy(VT) \\
%     %             else: \\
%     %                 M = np.concatenate((M, VT), 1) \\
                
%     %             VT = np.zeros((n*m,1), int) \\
%     % \Indm
%     % return M \\
%     % \Indm
%     %}
% % \pycode{   
% % def get\_dense\_class\_argmax(featmap, fc, gap, upsample=True):\\
% % \Indp
% %     \PyComment{featmap: n,c,h,w} \\
% %     \PyComment{fc: linear classifier operator} \\
% %     \PyComment{gap: spatial global average pooling operator} \\
% %     \PyComment{upsample: upsample featmap before getting dense class argmax} \\
% %     if upsample: \\
% %     \Indp
% %         featmap = F.upsample(featmap, scale\_factor=2., mode="bilinear") \\
% %     \Indm
% %     \\
% %     n, c, h, w = featmap.size() \\
% %     feat = featmap.permute(0, 2, 3, 1).reshape(n*h*w, c) \\
% %     logits = linear(featmap) \\
% %     dense\_logits = logits.reshape(n,h*w,-1) \\
% %     dense\_class\_argmax = dense\_logits.argmax(axis=2) \\
% %     \\
% %     return dense\_class\_argmax
% % \Indm
% % }
%     \PyComment{this is a comment} \\
%     \PyComment{} \\
%     \PyComment{going to have indentation} \\
%     \PyCode{for i in range(epochs):} \\
%     \Indp   % start indent
%         \PyCode{for (images,labels) in data\_loader:} \\
%         \Indp
%             \PyCode{logits=network(images)} \\
%             \PyComment{ignore the target class, n is the batch size and c is the number of class} \\
%             \PyCode{mask = torch.ones\_like(logits).scatter\_(1, labels.unsqueeze(1), 0.)} \\
%             \PyCode{logits\_non\_target = logits[mask.bool()].view((n, c-1))} \\
%             \PyCode{generate zipf\_dist from rank}\\
%             \PyCode{loss=CrossEntropy(logits,labels)+}
%             \PyCode{lambda*KLDiv(logits\_non\_target,zipf\_dist)}\\
%             \PyCode{loss.backward()}\\
%         \Indm
%     \Indm % end indent, must end with this, else all the below text will be indented
% \caption{PyTorch-style pseudo code for zipf's law soft label}
%\label{algo:your-algo}
%\end{algorithm}


Zipf's Label Smoothing aims to combine the best of the two worlds, the efficiency of teacher-free label smoothing and the informative soft label from self distillation. It generates non-uniform supervision signals from on-the-fly prediction of the network as shown in Fig. \ref{fig:overall framework}. Our method is inspired by the observation that the value and rank of the softmax output from the duly trained network  follow a distribution reminiscent to the Zipf's Law on average as shown in Fig. \ref{fig:prediction_zipf_fit}, which could be applied as a shape prior to the softmax prediction during the whole training period. To apply Zipf's Law to soft-label generation, ranking information of output categories is needed. We propose Dense Classification Ranking which utilizes local classification results to rank the categories. Finally, KL-divergence between prediction and Zipf's soft label within non-target classes is measured to provide more informative gradients for representation learning.

% Our motivation comes from finding that the output of the network obeys the Zipf's distribution. And we try to transfer this ``dark knowledge'' in an almost free manner.
% Our goal is to leverage an efficient label-smoothing regularization method of training, which is non-uniform and rank-relevant. In contrast of former knowledge distillation, our method requires no further more iterations or training data and requires little extra computation cost. The resulting Zipf's label smoothing is plug-and-play with common supervised learning. 
% The overall framework is shown in Fig.~\ref{fig:overall framework}.

\begin{figure*}[t]
  \centering
%   \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
  %\includegraphics[width=1.\textwidth,height=8cm]{figs/main3.png}
\includegraphics[width=1.\textwidth]{figs/main_1118.png}

  %\includegraphics{figs/main3.png}

  \caption{The overall Zipf's soft label generation and training framework. The blue dashed box outlines the soft label generation process. We apply a shared-classifier on dense feature maps and count the number of argmax values from the dense prediction, which could provide ranking information to Zipf's law distribution generation. For the non-occurred classes with zero count, we give uniform constant energy to them. $L_{zipf}$ is Kullback–Leibler divergence between the prediction of non-target classes and zipf's soft label, combined with $L_{CE}$ of the hard label to provide gradient to representation learning}
  \label{fig:overall framework}
\end{figure*}

\subsection{Zipf's Law}
Zipf's law is an empirical law which states that the normalized frequency of an element should be inversely proportional to the rank of the element, firstly discovered by G.Zipf on linguistic materials \cite{powers1998applications}. It can be described by an equation as:
\begin{equation} \label{zipf equation}
\begin{split}
    f(r) &= \frac{r^{-\alpha}}{\sum_{r=1}^{N} r^{-\alpha}}\\
    log f(r) &= -\alpha \log r - \log (\sum_{r=1}^{N} r^{-\alpha})\\
\end{split}
\end{equation}
where $r$ is the rank of the element, $N$ is the total number of elements, $f$ is the frequency and $\alpha$ is a constant larger than zero which controls the decay rate.

An interesting discovery is that the outputs of softmax networks follow Zipf's Law~\cite{powers1998applications} when the network is trained to its convergence state, and this pattern consistently emerges in different datasets and models as shown in Fig.~\ref{fig:prediction_zipf_fit}. We could exploit this shape prior to design a simple and efficient self-distillation algorithm. To generate a soft label using Zipf's distribution, ranking information of categories is a must which is almost impossible to get from annotation.
% As shown in Figure~\ref{fig:prediction_zipf_fit}, when a network is trained to its convergence state, the average distribution of sorted softmax values follows Zipf's law well.
%predictions from three major classification data sets are averaged among samples and sorted along the axis of categories, which appear approximately linear on a log-log graph respectively. 
% So we use Zipf's soft labels as an extra supervision.
% So replacing one-hot encoding labels with generated Zipf's soft labels to boost performance seems to be a better option.
%In this paper we focus on how to generate soft labels from free dark knowledge during training. 
% The construction of our Zipf's label smoothing involves a sample-wise ranking of classes and the Zipf's loss, as introduced in the following.

% \subsection{Zipf's Law}
% Zipf's law is an empirical law which states that the normalized frequency of an element should be inversely proportional to the rank of the element, firstly discovered by G.Zipf on linguistic materials \cite{powers1998applications}. It can be described by an equation as:
% \begin{equation} \label{zipf equation}
%     f(k) = \frac{k^{-\alpha}}{\sum_{n=1}^{N} n^{-\alpha}}
% \end{equation}
% where $k$ is the rank of the element, $N$ is the total number of elements, $f$ is the frequency and $\alpha$ is a constant larger than zero. The relation between the frequency and $k$ appears linear on a log-log graph:
% \begin{equation} \label{log zipf equation}
%     \log f(k) = -\alpha \log k - \log (\sum_{n=1}^{N} n^{-\alpha})
% \end{equation}



% % We discovered that the output of a deep neural network trained for a classification task follows the law as well. The sorted value of soft-max predictions of a sample appears a well-regulated pattern with the rank of classes. As shown in Figure \ref{fig:prediction_zipf_fit}, predictions from three major classification data sets are averaged among samples and sorted along the axis of categories, which appear approximately linear on a log-log graph respectively. The rank of classes can also be calculated from the similarity between the target class (ground truth label) and other non-target classes or the likelihood that a sample is classified to a class.
% We discover that the sorted softmax output of a deep neural network trained for a classification task follows the law as well. As shown in Figure \ref{fig:prediction_zipf_fit}, sorted probabilities averaged across samples appear approximately as a linear line on a log-log graph with respect to the rank. This relationship holds regardless of the datasets and models we use. Hence, it suggests a good prior to be used to regularize the distribution of non-target class probability during training.

\subsection{Dense Classification Ranking}\label{spatial-dense vote rank}
% To parameterize Zipf's distribution for each sample during training, we should give ranks to non-target class according to some metrics. During the training process, deep neural networks are supposed to have probable potential to learn the likelihood of other non-target classes along with the target class. Therefore, the prediction of every instance itself provides the value for ranking. Then the rank can be used to generate a power-law shape distribution to regularize non-target class learning. 

To realize the Zipf distribution we need to find a way to properly rank the output categories. The naive thought is to directly sort the softmax prediction of a sample, which we call the logit-based ranking method. Though this method already generates performance gain (as shown in section~\ref{section:ablation}), we find a finer treatment of the relative ranking of the top classes to be beneficial.

% The idea is that network is often capable of generating dense classification labels from the last few layers before the global average pooling (as exploited in the CAM visualization~\cite{zhou2016learning} etc.).\\

% However, since only the one-hot supervision is imposed during training, we can hardly get reliable ranking information from that, especially in the tail of ranking when the category number of classes is large.
%However, the values of tail class predictions are suppressed during the training process, which leads to a very noisy signal of the ranks. Therefore, it is reasonable that only a few reliable top ranking categories can be obtained from the sample itself, and uniform distribution should be a more proper choice for the remaining categories. Besides, there are some non-target objects spatially shown along with the target on most images, and it's irrational to suppress predictions of these non-target classes during training. We can get the corresponding local label by applying classifier on the dense feature map. Counting the argmax values of predictions from dense feature map can be served as a ranking metric.

% the fluctuation of low-rank class predictions during the training process results a very low signal-to-noise ratio (SNR) of ranks, especially in the tail of the ranking.
% making it unreliable to fit an zipf's distribution for low-rank class predictions. Besides, the accuracy of classification suffers from the disturbing overlapping objects in the background, making networks hard to predict whether the object is to be classified in some circumstances.
% \par
% To address these problems, we proposed a ranking method called the spatial-dense vote rank.
% \subsubsection{Logits rank}
% \par
% We have a dataset $ S=\{(x_1, y_1), ..., (x_N, y_N)\} \subset (X, Y^h)$, where X represents the input space and the $ Y^h $ represents the hard-label space for which each label is encoded into one-hot vector. $ x_i $ in input space is transformed to $ f_i $ by non-linear neural network $ F_\theta $, and then features $ f_i $ are transformed to logits $ z_i $ using fully-connected linear mapping $ FC $ and global average pooling ($GAP$). At last $ Softmax $ is applied to gain classes distribution $ p_i $, where $ p_i $ is a vector length of class number $ C $:
% \begin{equation}\label{logit_rank}
% \begin{split}
% f_i &= F_\theta(x_i) \\
% z_i &= FC(GAP(f_i)) \\
% p_{i} &= Softmax(z_{i}),    j=1,2,...,C
% \end{split}
% \end{equation}
% Therefore, the class $j$ rank of instance $ x_i $ should be:
% \begin{equation} \label{logit_rank_1}
% \begin{split}
% rank_{ij} &= rank(p_{ij}),    j=1,2,...,C
% \end{split}
% \end{equation}
% \par
% The output vector for each instance can have different kinds of meanings from different perspectives. $ p_{ij} $ does not only demonstrate the extent of how likely the sample  $ x_i $ belongs to class $j$ but also describes the similarity between the ground truth class and any other class $j$ on $ x_i $. For example, an image of a cat is more likely to have a higher prediction on class "dog" instead of class "chair". 
%\subsubsection{Spatial-dense vote rank} 


% \noindent \textbf{Dense classification ranking.} 
Common image classification convolution networks extract a feature map $\boldsymbol{F}$ from an image sample. A global average pooling ($GAP$) is then applied to $\boldsymbol{F}$.
% adapt with different image and feature sizes. 
The fully-connected layer ${FC}$ and soft-max operation will output the logits $\boldsymbol{z}$ and the final prediction $\boldsymbol{p}$.

% As shown in Figure \ref{fig:overall framework}, global feature $\boldsymbol{f}$ of an sample $(\boldsymbol{x},y)$ from the data set $\{(\boldsymbol{x_1},y_1),(\boldsymbol{x_2},y_2),...,(\boldsymbol{x_N},y_N)\}$ is extracted from an convolution network backbone $F_\boldsymbol{\theta}$ followed by global average pooling ($GAP$) operation. ${FC_\boldsymbol{\phi}}$ is one fully-connected layer, which could be applied on global feature $\boldsymbol{f}$ to get logits $\boldsymbol{z}$ and global prediction $\boldsymbol{p}$ as:
% Since $GAP$ is a scaling operation on spatial dimension, we could also 
% Instead of using global average pooling on spatial feature $\boldsymbol{f}$ like normal classification network, we apply an spatial-wise fully-connected linear mapping $ FC $ on every spatial location of $\boldsymbol{f}$ to get spatial-dense logits $\boldsymbol{z}$  and prediction $\boldsymbol{p}$ by:
% \begin{equation} \label{global_eq}
% \begin{split}
% \boldsymbol{f} &= GAP(F_\theta(\boldsymbol{x})) \\
% \boldsymbol{z} & = FC_\phi(\boldsymbol{f}))\\
% \boldsymbol{p} &= Softmax(\boldsymbol{z})\\
% \end{split}
% \end{equation}
%\par
% We denote $\boldsymbol{p}(c|\boldsymbol{x})$ is the predicted probability of a class $c$ for an sample $\boldsymbol{x}$. We write $\boldsymbol{p}(c|\boldsymbol{x})$ as $\boldsymbol{p}(c)$ for simplicity.
%\par
If we used ${FC}$ directly on every pixel of the dense feature map $\boldsymbol{F}$, we cat get local classification results  $\boldsymbol{p}^{L}$:

% Instead of using GAP before fully connected layer to get global feature, we used ${FC}$ directly on every pixel of the dense feature map $\boldsymbol{F}$ to get pixel-wise dense local predictions $\boldsymbol{p}^{L}$:
% the classifier ${FC_\phi}$ could be applied locally on  $\boldsymbol{f_k}$ to get prediction $\boldsymbol{p_k}$ from each position $k$ in dense feature map as:
\begin{equation} \label{local_eq}
\begin{split}
% \boldsymbol{z}_k^{local} &=FC_\phi(\boldsymbol{f}_k),  k=1,2,...,K\\
\boldsymbol{p}_k^{L} &= Softmax(FC_\phi(\boldsymbol{F}_k)), k=1,2,...,H\times W\\
\end{split}
\end{equation}
\par
where $L$ is just a mark to show the difference between global prediction $\boldsymbol{p}$ and local predictions $\boldsymbol{p}^L$. These predictions give a more complete description of what the image contains, as the object of the target class usually only occupies part of the image. We take this information into account by identifying the individual top-1 class from each location as a vote and aggregate the votes into a histogram. The classes are finally ranked by their frequency of appearance in the histogram. The remaining classes will share the same lowest rank.

% As for small size images (e.g. $32\times 32$ in CIFAR), we find that a minimum amount of votes is required for our method to distinguish different classes. So we use variants of the backbone that also have class supervision on feature maps with higher resolution than the last one. Votes may be gathered from multiple layers so that a meaningful rank could be constructed.
% A consequence of this voting-based method may be that we have to clip the Zipf's values to a uniform one after a certain rank, as they would not receive sufficient votes to be distinguished individually. 
% However, the logit-based ranking method suffers from the fluctuation of low-rank class predictions during training and result in a low signal-noise ratio on low ranks. A uniform same rank can equally contribute to low-rank classes.

% \begin{equation} \label{rank}
% \begin{split}
% \boldsymbol{vote}(c) &= \sum_{k=1}^{K}\delta_{c}(\mathop{\arg\max}\limits_{m \in \left \{1,2,...,C\right\}}\boldsymbol{p}_k^{L}(m)) \\
% \delta_{c}(n) &=\delta(n-c) =\begin{cases}
% 1, &n=c \\
% 0,&n \neq c \\
% \end{cases},c = 1,2,...,C\\
% \end{split}
% \end{equation}
%\boldsymbol{vote}_{c} &= \sum_{k=1}^{K}\delta_{c}(\arg\max\boldsymbol{p_k}), \\

%c &\in \left \{1,2,...,C\right\}\\

% where $\boldsymbol{p_k}_{m}$ is the probability of class $m$ on spatial location $k$ and $C$ is the class number of the data set. $\delta_{c}(n)$ is an discrete Dirac-delta function with an off-set $c$. The final ranks can be generated by:\\
% \begin{equation}
% \boldsymbol{r} = Rank(\boldsymbol{vote})\\
% \end{equation}

% $Rank$ is a function which assign ranks to votes. We denote $\boldsymbol{r}_c$ is the rank of class $c$. The classes which get zero votes share the same last rank, leading to an uniform distribution for the tailing classes.  \\



% \begin{equation} \label{Dirac-delta}
% \begin{split}
% \delta_{c}(n) &=\delta(n-c) =\begin{cases}
% 1, &n=c \\
% 0,&n \neq c \\
% \end{cases}\\
% \end{split}
% \end{equation}

% \par
% Only the top-1 non-target class of the prediction is considered during our spatial-dense vote rank by the operation of $\arg \max$ due to the low signal-to-noise ratio of spatial ranks. Without global average pooling, the receptive field becomes smaller than the whole image. It only gives prediction based on the local information, making the spatial ranks unreliable. However, we discovered that the top-1 class is still accurate spatially and finding $\arg \max$ is more time-efficient than sorting the logits when class number $C$ of data sets, i.e. fine-grained data sets, is huge. 
% \par
% Another advantage of our spatial-dense vote rank is that it can decide dynamically how many ranks are reliable of generating Zipf's law distribution soft label by the total number of classes which get more than zero votes from the spatial dimension. Meanwhile, the classes which get zero votes have a trivial influence on soft-max predictions hence they share the same lowest rank in the Zipf's law.

\subsection{Zipf's Loss}
% After the soft label distribution observation in Fig. \ref{fig:prediction_zipf_fit}, we conjecture that prior Zipf's-law distribution $\tilde{p_i}$ applys for non-target classes and could be imposed as a regularization early during training. 
Zipf's loss $L_{Zipf}$ of image sample $\boldsymbol{x}$ and label $y$ is defined as KL-divergence $D_{KL}$ between normalized non-target prediction $ \boldsymbol{\hat{p}} $ and the synthetic Zipf's soft label $ \boldsymbol{\tilde{p}}$ generated from dense classification ranking:

\begin{equation} \label{eq_KL_zipf}
\begin{split}
\boldsymbol{\hat{p}}_c&=\frac{\exp{(\boldsymbol{z}_{c})}}{\sum_{m=1,m\neq y}^{C}{\exp{(\boldsymbol{z}_{m})}}}\\
% =\frac{\boldsymbol{p}(c)}{1-\boldsymbol{p}(y)},\\
L_{Zipf}(\boldsymbol{x},y) &= D_{KL}(\boldsymbol{\tilde{p}}||\boldsymbol{\hat{p}}) =\sum_{c=1,c\neq y}^{C} \boldsymbol{\tilde{p}}_c log \frac{\boldsymbol{\tilde{p}}_c}{\boldsymbol{\hat{p}}_c} \\
\end{split}
\end{equation}
\par

The synthetic Zipf's label $\boldsymbol{\tilde{p}}$ of non-target class $c$ should follow the equation \ref{prob_zipf} of Zipf's law with the corresponding rank $\boldsymbol{r}_c$:

% and they can be determined by the ranks from the current prediction. We form the spatial-dense vote ranks as we described in Section \ref{spatial-dense vote rank}. The target class is included during spatial-dense vote rank, and excluded during the generation of Zipf's-law distribution. 


\begin{equation} \label{prob_zipf}
\begin{split} 
    \boldsymbol{\tilde{p}} _c&= \frac{{\boldsymbol{r}_{c}}^{-\alpha}}{\sum_{m=1,m\neq y}^{C} {\boldsymbol{r}_{m}}^{-\alpha}} \\
\end{split}
\end{equation}
\par

where $\alpha$ is a hyper-parameter that controls the shape of the distribution.
% However,  this zipf's law generated distribution drastically changes along with the number of classes $C$, making it hard to fit all kinds of datasets. We assume that certain percentage of top rank classes should have certain amount of energy in distribution $ \tilde{p_i} $. 
% Therefore an probability density function of rank is introduced and the unbiased distribution can be generated from it:
% \begin{equation} \label{prob_unbias_zipf}
% \begin{split} 
%     pdf(x) &=\frac{1}{x^\alpha}\\
%     \tilde{p_{ij}}_{unbias} &=\int_{lb+interval*(rank(j)-1)}^{lb+interval*(rank(j))} pdf(x) dx \\
%     interval &=\frac{rb-lb}{C}\\
% \end{split}
% \end{equation}
% where $rb$ is the constant of right integral bound and $lb$ is the left integral bound. We call it unbiased zipf's law distribution.



The $L_{CE}$ is the standard cross entropy loss with one-hot ground-truth label. The combined loss function is as follow:
\begin{equation} \label{eq_KL_totalloss}
\begin{split}
Loss(\boldsymbol{x},y) =L_{CE}(\boldsymbol{x},y)+\lambda L_{Zipf}(\boldsymbol{x},y)
\end{split}
\end{equation}
$L_{CE}$ encourages the prediction to be sharp and confident in the target class, while $L_{Zipf}$ regularized the prediction to be soft within non-target classes.$\lambda$ is a hyper-parameter which control the regularization strength.


\noindent \textbf{Comparison with Uniform Label Smoothing.}
The gradient with respect to non-target logits for $L_{zipf}$ and ${L_{LS}}$ are shown as:

\begin{equation}\label{gradient}
\begin{split}
\frac{\partial L_{Zipf}(\boldsymbol{x},y)}{\partial \boldsymbol{z}_{c}}
 &= \begin{cases}
0 &\text{$c = y$}\\
\boldsymbol{\hat{p}}_c-\boldsymbol{\tilde{p}}_c &\text{$c \neq y$}
\end{cases} \\
\frac{\partial L_{LS}(\boldsymbol{x}, y)}{\partial \boldsymbol{z}_{c}}
 &= \begin{cases}
\boldsymbol{p}_c - (1-\beta) &\text{$c = y$}\\
\boldsymbol{p}_c - \frac{\beta}{C-1} &\text{$c \neq y$}
\end{cases} \\
\end{split}
\end{equation}

Label smoothing generates a soft label with a uniform value $\frac{\beta}{C-1}$ for all non-target classes and $1-\beta$ for the target class, where $C$ is the total number of classes. However, label smoothing suppresses predictions of high-ranked classes or promotes predictions of low-ranked classes to the same level since $\beta$ is constant and rank-irrelevant, which is conceptually sub-optimal. 

Our Zipf's loss is rank-relevant compared with label smoothing. In non-target classes, it encourages the high-ranked classes to keep larger predictions than low-ranked ones. Zipf's law distribution shows empirical success in our experiments against other rank-relevant distributions such as linear decay, more details are shown in Section \ref{sec:ablation study}.

% Zipf's law constrained soft label, however, solved this problem partially. For the $L_{Zipf}$ loss, the graidents respect to logits $z_j$ are


% \subsection{Mathematics}
% In this section, we will first give a formal definition of the problem. Afterward, the proposed algorithm is described, and further analyses are provided to support the claim.

% \subsubsection{problem statement}
% We have a dataset $ S=\{(x_1, y_1), ..., (x_N, y_N)\} \subset (X, Y^h)$, where X represents the input space and the $ Y^h $ represents the hard-label space for which each label is encoded into one-hot vector. Our goal is soften the hard label using emerging knowledge during training to improve representation learning. 

% $ x_i $ in input space is transformed to $ f_i $ by non-linear neural network $ F_\theta $, and then features $ f_i $ are transformed to logits $ z_i $ using fully-connected linear mapping $ FC $, and at last $ Softmax $ is applied to gain classes distribution $ p_i $, where $ p_i $ is a vector length of class number $ C $. In naive one-pass training, $ F_\theta $ is optimized by loss function such as cross-entropy during training, but the sub-optimal hard label supervision make it difficult to capture non target class relationship.
% \begin{equation}
% \begin{split}
% f_i &= F_\theta(x_i) \\
% z_i &= FC(f_i) \\
% p_i &= Softmax(z_i) 
% \end{split}
% \end{equation}

% \subsubsection{zipf's law constrained soft label}
% Zipf's law  is an empirical law formulated using mathematical statistics that refers to the fact that for many types of data studied in the physical and social sciences, the rank-frequency distribution is an inverse relation.\cite{zipf}. Zipf's law is a common pattern in nature or human society, also We zipf's law like class distribution for several popular backbones after training, thus we conjecture this pattern happen in non target class distribution for each sample during training too, which we can exploit to generate soft label to replace hard label for better representation learning.

% Inspired by zipf's law, we conjecture that prior distribution $ \tilde{p_i} $ exist in non-target classes, and they can be determined by the ranks from the current prediction. For a sample $(x_i, y_i^h)$, prior distribution $\tilde{p_i}$ for each of the non-target classes can be determined by the \ref{eq_prob_zipf}.
% \begin{equation} \label{eq_prob_zipf}
% \begin{split} 
%     log(\tilde{p_{ij}}) &= -alpha * log(Rank(p_{ij})) + Const  \\
%     Rank(p_{ij}) &\in \{1, ..., C-1\} \\
%     j &\in [0, C-1] \backslash {y_i^h} 
% \end{split}
% \end{equation}

% % \begin{figure}[t]
% %   \centering
% % %   \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
% %   \includegraphics[width=0.8\linewidth]{figs/overrall.png}

% %   \caption{Example of caption.
% %   It is set in Roman so that mathematics (always set in Roman: $B \sin A = A \sin B$) may be included without an ugly clash.}
% %   \label{fig:onecol}
% % \end{figure}

% $ Rank $ is a function which assigns ranks to probabilities in non-target classes. $ alpha $ is larger than zero, the larger the $ alpha $ is, the more concentrated the probabilities would be in the top few non-target classes. 


% \subsubsection{zipf's law constrained KL-divergence}
% With the soft probabilities supervision constrained by zipf's law, We could use the common KL-divergence to measure the distance between current prediction $ P_{ij} $ and the prior distribution $ \tilde{P_{ij}} $ from zipf's law. 

% \begin{equation} \label{eq_KL_zipf}
% \begin{split}
% KL_{zipf}(x_i) =\[ \sum_{j=0,j!=y_i^h}^{C-1} \tilde{p_{ij}} log \frac{\tilde{p_{ij}}}{p_{ij}} \]
% \end{split}
% \end{equation}


% Our soft distribution is rank-relevant compared with label smoothing. It encourages more to high-ranked classes with a higher probability generated from Zipf's distribution and suppresses the contrary since higher the rank is, more likely the sample belongs to the class. We tolerate the differences between predictions of different non-target classes instead of optimizing it to a constant (0 in the cross-entropy case, and $\frac{\alpha}{C-1}$ in the label smoothing case). And the total loss combined by hard label cross-entropy loss and Zipf's loss guarantees that the target class has priority and  any non-target class cannot be supreme in any circumstance during the training process.


% \subsection{combined loss}

% the combined loss is written as:
% \begin{equation}\label{eq_combine_loss}
% Loss = Loss_{xent}(x_i, y_i^h)} + \lambda * KL_{zipf}
% \end{equation}



% \subsection{generate rank during training}

% compare different rank methods




==> related_work.tex <==
\subsection{Label Smoothing}
The one-hot label is sub-optimal because objects from more than one class occur in the same image.
Label Smoothing~\cite{szegedy2016rethinking} (LS) is proposed to smooth the hard label to prevent over-confident prediction and improve classification performance.
% M{\"u}ller et al.~\cite{muller2019does} found that the feature of training examples from the same class gather in tighter clusters when LS is used, which improves generalization.
M{\"u}ller et al.~\cite{muller2019does} found that intra-class distance in feature space is more compact when LS is used, which improves generalization.
To obtain non-uniform soft labels, Zhang et al.~\cite{zhang2021delving} proposed the online label smoothing method (OLS) by maintaining the historical predictions to obtain the class-wise soft label. Yuan et al.~\cite{yuan2020revisiting} discussed the relationship between LS and knowledge distillation, and proposed a teacher-free knowledge distillation (Tf-KD) method to get better performance than LS. Label smoothing has become one of the best practices in the current deep learning community~\cite{he2019bag}, but the paradigm of using uniform distribution for the non-target classes limits further improvement of performance. 

\subsection{Knowledge Distillation}
Instead of imposing a fixed prior distribution, knowledge distillation was first proposed by Hinton in~\cite{hinton2015distilling} to provide sample-level non-uniform soft labels. They demonstrated that the ``dark knowledge'' lies in the output distributions from a large capacity teacher network and benefits the student's representation learning. 
Recent works mainly explored to better transfer the ``dark knowledge'' and improve the efficiency from various aspects, such as reducing the difference between the teacher and student~\cite{cho2019efficacy, mirzadeh2020improved, zhu2021student, beyer2021knowledge}, designing student-friendly architecture~\cite{park2021learning, Ma2021UndistillableMA}, improving the distillation efficiency~\cite{kim2021self, furlanello2018born, xu2019data, yun2020regularizing} and explaining the distillation's working mechanism~\cite{stanton2021does, allen2020towards}.

In this work, we focus on how to transfer the ``dark knowledge'' in an almost free manner.
% In fact, the larger teacher is not a must-have option.
Furlanello et al.~\cite{furlanello2018born} proposed to improve the performance of the student network by distilling a teacher network with the same architecture.
However, it is still a two-stage approach, which first trains the teacher and then distills knowledge to the student. To reduce the training time, many self-distillation methods were proposed. They gain soft label supervision on the fly without the pretraining step.

\subsection{Self Distillation}
There are two categories of self-distillation techniques, namely the auxiliary parameter methods~\cite{guo2020online, zhang2019your, bagherinezhad2018label, ji2021refine, zagoruyko2016paying} and contrastive sample  methods~\cite{xu2019data, yun2020regularizing, zhang2021delving, kim2021self}. Auxiliary model methods exploit additional branches to get extra predictions besides the main-branch prediction for soft label supervision at the cost of more parameters overhead. For example, Knowledge Distillation via Collaborative Learning (KDCL)~\cite{guo2020online} trained multiple parallel student networks at the same time and ensemble the output as extra soft label supervision for each parallel student network. On the other hand, contrastive sample methods get soft label supervision at the cost of additional data augmentation, enlarged batch size, or complex sampling strategy. The examples are Data-distortion Guided Self-Distillation (DDGSD)~\cite{xu2019data} which gains soft labels from different augmented views from the same instance and Regularizing Class-wise Predictions via Self-knowledge Distillation (CS-KD)~\cite{yun2020regularizing} which gathers data from other samples of the same class.

As summarized above, Label Smoothing and Knowledge Distillation are two major techniques to acquire informative soft labels. However, the Label Smoothing methods are limited by the uniform hypothesis, while the Knowledge Distillation methods require much more memory or computation overhead. Our work aims to improve upon these issues.


% To remove the requirement of the teacher, teacher-free methods gain soft label supervision on the fly, which could reduce the training time budget and achieve almost the same or even more performance gains. There are two categories of these methods. The first is the multi-branches method, which uses a multi-branches structure to get different predictions. The second is the cross-batch stats method, which maintains global statistics from all predictions or exploits feature consistency between samples within a local minibatch or different views from a single sample.

% Multi-branches methods exploit or ensemble predictions from other branches as soft labels at the cost of more parameters during training. Be Your Own Teacher (BYOT)\cite{zhang2019your} train multiple classifiers at different depths using the prediction from the deepest layer as soft label supervision. Knowledge distillation via collaborative Learning (KDCL)\cite{guo2020online} train multiple parallel student networks at the same time, and ensemble the output as extra soft label supervision for each parallel student network. 



% Cross-batch stats methods maintain global statistics, or using cross-batch statistics to gather class-level or sample-level soft-labels, at the cost of data augmentation, large batch size or complex sampling strategy. Data-distortion guided self-distillation(DDGSD)\cite{xu2019data} gains soft labels from different augmented views from the same instance. Regularizing Class-wise Predictions via Self-knowledge Distillation (CS-KD)\cite{yun2020regularizing} gains soft label from other samples of the same class in the a local minibatch. Online label smoothing method (OLS)\cite{zhang2021delving} maintains the historical predictions from different classes to obtain class-level not sample-level soft label. 


% Zhang et al.~\cite{zhang2021understanding} find an interesting phenomenon that even random labels can be fitted easily.
%Xie et al.~\cite{xie2016disturblabel} disturb the labels to prevent over-fitting.
% Soft label has also been used in many unsupervised domain adaption tasks.
% Zou et al.~\cite{zou2018unsupervised} apply pseudo-labels to the top k\% of each category of the target domain to improve the label accuracy. They further propose confidence regularization and model regularization to improve the performance~\cite{zou2019confidence}.

% \subsection{Label refinery}
% Even though the label smooth technique is a good regularization method and can prevent the over-confidence phenomenon, some studies point out that 

% Methods focus on the refinery of labels through additional architectures or samples~\cite{bagherinezhad2018label, li2017learning, wu2017hierarchical, wu2018multi, cai2007exploiting}. 
% Despite using soft label regularization, some researchers try to refine the labels.
% Bagherinezhad et al.~\cite{bagherinezhad2018label} propose an iterative method to refine the soft labels during training.
% Li et al.~\cite{li2017learning} design a framework to learn from noisy labels incorporating with a knowledge graph, which can improve the quality of the labels.
% Wu et al.~\cite{wu2017hierarchical} propose a hierarchical loss based on an ultrametric tree with semantical meanings.
% Wu et al.~\cite{wu2018multi} use mixed dependency graphs to learn with missing labels.
% Cai et al.~\cite{cai2007exploiting} incorporate the category taxonomy into the learning architecture and design a hierarchical loss for overlapping categories.
%Some researchers try to re-label the samples directly through a stronger classifier or even manual annotation~\cite{beyer2020we, shankar2020evaluating, yun2021re}.
% Considering that many classification tasks contain multiple labels and erroneous single labels, some researchers try to re-label the samples.
% Beyer et al.~\cite{beyer2020we} investigate recent studies on ImageNet and find that some studies may be meaningless due to the incorrect labels.
% Shankar et al.~\cite{shankar2020evaluating} propose to refine the validation labels into multiple labels.
% Yun et al.~\cite{yun2021re} re-label the ImageNet labels of multiple and localized labels by a stronger classifier.


% We demonstrate that Zipf's law can perform better than previous hand-crafted distributions and require little computation overhead, which is a simple and effective assumption to better model the soft label distributions. 

% Ji et al.~\cite{ji2021refine} propose to teach the student network from itself. A teacher network is learned from some auxiliary layers.
% Zhang et al.~\cite{zhang2019your} propose a self distillation method to supervise the shallow layers with deep layers.
% Reed et al.~\cite{reed2014training} propose to handle the noisy labels through prediction consistency by a bootstrapping method.
% Inspired by the successful use of low entropy penalty in reinforcement learning, Pereyra et al.~\cite{pereyra2017regularizing} penalize the output distributions to improve the classification performance. 

% Some studies further demonstrate better results by distilling the dark knowledge from all aspects, such as intermediate layers~\cite{romero2014fitnets}, attention maps~\cite{zagoruyko2016paying}, the relationship between intermediate layers~\cite{yim2017gift} and the similarity between samples of the same class~\cite{yun2020regularizing}.

%Zhu et al.~\cite{zhu2021complementary} introduce metric learning into distillation and propose to distill the relationship between the samples.
% Romero et al.~\cite{romero2014fitnets} further distill the dark knowledge from the intermediate layers.
% Zagoruyko et al.~\cite{zagoruyko2016paying} distill the dark knowledge from the attention maps.
%Gou et al.~\cite{gou2021knowledge} have surveyed to introduce recent works of knowledge distillation. It consists of knowledge representation, teacher-student architecture, and distilling methods. 
% Yim et al.~\cite{yim2017gift} propose to distill knowledge from the relationship from intermediate layers and acquire better results than simple soft labels.
% Yun et al.~\cite{yun2020regularizing} introduce class-wise knowledge distillation to penalize the similarity between samples of the same class,  which reduces the intra-class variance and acquires more meaningful results. 
% Zhu et al.~\cite{zhu2021complementary} introduce metric learning into distillation and propose to distill the relationship between the samples.

% \subsection{Self-knowledge distillation}
% Although the above methods have acquired better soft labels, they all need additional models or larger computation overhead.
% To get rid of the dependence on large models, many self-knowledge distillation methods are proposed.
% Different from normal distillation that transfers knowledge to a smaller network, Furlanello et al.~\cite{furlanello2018born} propose to improve the performance of the student network by distilling from a teacher network with the same architecture.
% Ji et al.~\cite{ji2021refine} propose to teach the student network from itself. A teacher network is learned from some auxiliary layers.
% Zhang et al.~\cite{zhang2019your} propose a self distillation method to supervise the shallow layers with deep layers.
% Reed et al.~\cite{reed2014training} propose to handle the noisy labels through prediction consistency by a bootstrapping method.
% Inspired by the successful use of low entropy penalty in reinforcement learning, Pereyra et al.~\cite{pereyra2017regularizing} penalize the output distributions to improve the classification performance. 
% Miyato et al.~\cite{miyato2015distributional} propose the local distributional smoothness to disturb the input while maintaining the output's consistency. The model generalization is prompted by an adversarial method.

% As summarized above, label smooth and knowledge distillation are two major techniques to acquire better soft labels. However, the label smooth methods are limited by the uniform hypothesis, while the knowledge distillation methods require a large computation overhead.
% We demonstrate that Zipf's law can perform better than previous hand-crafted distributions and require little computation overhead, which is a simple and effective assumption to better model the soft label distributions. 
% Different from classic knowledge distillation methods that require big models, self-knowledge distillation is faster and more convenient to use. 

